Camera clustering for scalable stream-based active distillation

We present a scalable framework designed to craft efficient lightweight models for video object detection utilizing self-training and knowledge distillation techniques. We scrutinize methodologies for the ideal selection of training images from video streams and the efficacy of model sharing across numerous cameras. By advocating for a camera clustering methodology, we aim to diminish the requisite number of models for training while augmenting the distillation dataset. The findings affirm that proper camera clustering notably amplifies the accuracy of distilled models, eclipsing the methodologies that employ distinct models for each camera or a universal model trained on the aggregate camera data.

==> 1_Abstract/abstract_journal.tex <==
We present a scalable framework designed to craft efficient and lightweight models for video object detection, utilizing self-training and knowledge distillation techniques. We scrutinize methodologies for the ideal selection of training images from video streams and the efficacy of model sharing across numerous cameras. By advocating for a camera clustering methodology, we aim to diminish the requisite number of models for training while augmenting the distillation dataset. The findings affirm that proper camera clustering notably amplifies the accuracy of distilled models, eclipsing the methodologies that employ distinct models for each camera or a universal model trained on the aggregate camera data.




==> 4_SOTA/archives/AL_sota_cvpr.tex <==
\subsection{Active Learning}
AL-based sampling schemes are used to minimize the number of labels required for training a model by selecting the most informative data points \cite{Settles2009}. AL can be broadly categorized into three macro scenarios, membership query synthesis, pool-based AL, and stream-based AL \cite{surveyOAL}. In the context of deep AL, the majority of the approaches have been focused on the second scenario, which depicts a static scenario where the learner must select the most useful data points from a closed set of unlabeled observations. To the best of our knowledge, the stream-based AL scenario for object detectors has never been investigated. In computer vision, despite a recent spark of interest in object detection-oriented sampling schemes, most of the AL strategies have been developed for image classification tasks. Another key characteristic of AL is that it generally assumes the availability of a perfect oracle. That is, whenever a data point is queried, its true label is revealed. Unfortunately, this assumption does not hold in a KD framework, where the pseudo-labels provided by the teacher might prove wrong.

\paragraph{Active Learning for Image Classification.} Many AL strategies have been proposed for pool-based AL for classification, and they can mostly be classified into uncertainty-based or diversity-based approaches \cite{WuEntropy}. Among the uncertainty-based strategies, a very common strategy is to estimate the model uncertainty using Monte-Carlo (MC) dropout \cite{Gal2017} or ensemble networks \cite{Mohamadi}. Entropy and margin-based sampling strategies are also widely employed \cite{5206627,Roth2006}. Learn loss \cite{Yoo2019} is a task-agnostic method that introduces a loss prediction module to the network, which is used to estimate the data points that are likely to be wrongly predicted. Among the diversity-based strategies, Core-set \cite{Sener2017} is one of the most popular strategies, and it uses a k-centre-Greedy algorithm to locate a set of representative data points. Cluster-Margin \cite{Citovsky2021} further extends Core-set by combining uncertainty and diversity. Margin and diversity are also taken into account in the DRMRS strategy proposed by Elhamifar et al. \cite{Elhamifar2013}. BADGE \cite{Ash2019} strikes a balance between uncertainty and diversity by using a $k-$\asc{MEANS++} seeding algorithm on the gradients obtained from the last layer of the network. CDAL \cite{Agarwal2020} leverages the K-center-Greedy algorithm used in Core-set, replacing the Euclidean distance with the pairwise contextual diversity. CLUE \cite{Prabhu} performs uncertainty-weighted clustering to identify target instances that are both uncertain according to the model and diverse in feature space. VAAL \cite{sinha2019variational} uses a VAE to map the instances into a latent space, which is then fed into a discriminator that learns to differentiate between the labeled data already available and the unlabeled samples.

\paragraph{Active Learning for Object Detection.} Roy et al. \cite{RoyUnmesh} classified active learning approaches for single-shot multi-box detectors into two categories, black-box methods that do not depend on the underlying network architecture and use informativeness scores as the confidence obtained from the softmax layer, and white-box methods are dependent on the architecture of the underlying network. Among the black-box methods, the authors suggested using the minmax approach, which selects the least confident images among the unlabeled pool. According to this strategy, the confidence of an image is given by the maximum confidence score between the detected bounding boxes. Different aggregation functions for the confidence scores have also been explored \cite{Brust2018,Probst2022}. Ensemble methods have also been used for object detection-oriented AL \cite{FengDi,Schmidt2020}. Kao et al. \cite{Kao2018} proposed a query strategy based on localization tightness and stability. Choi et al. \cite{DBLP:journals/corr/abs-2103-16130} proposed a probabilistic framework based on mixture density networks. CALD \cite{WeipingYu} unifies box regression and classification within a single metric, taking into account the consistency between original and augmented images. MIAL \cite{Yuan2021} is a multiple-instance framework that bridges the gap between the instance-level and image-level uncertainty by filtering out noisy instances. PPAL \cite{Yang2022} is a two-stage algorithm that includes difficulty-calibrated uncertainty sampling and category-conditioned matching similarity. Aghdam et al. \cite{Aghdam2019} proposed a new function that aggregates the pixel-level scores to estimate the uncertainty of background pixels. Huang et al. \cite{Huang2022} proposed a method for selecting images based on their frequency domain values, which are calculated using a Fourier Transform. 


==> 4_SOTA/archives/AL_sota_cvpr_short.tex <==
\subsection{\acl{AL}}

\ac{AL} is a sampling approach that selects the most informative data points to minimize the number of labels required for model training \cite{Settles2009}. \ac{AL} can be divided into three macro scenarios: synthesis of membership queries, pooled \ac{AL}, and streamed \ac{AL} \cite{surveyOAL}. The majority of approaches in deep \ac{AL} have focused on the pool-based scenario, where the learner selects the most useful data points from a closed set of unlabeled observations. \ul{The stream-based AL scenario for object detectors has not been investigated}. Moreover, \ac{AL} assumes the availability of a perfect oracle, where the true label of a data point is revealed when queried. However, this assumption does not hold in a \ac{KD} framework, where the pseudo-labels provided by the teacher may be incorrect.

\paragraph{\acl{AL} for Image Classification.} \acs{AL} strategies for pool-based classification can be categorized into uncertainty-based or diversity-based approaches \cite{WuEntropy}. Uncertainty-based strategies estimate model uncertainty using techniques such as Monte Carlo dropout \cite{Gal2017} or ensemble networks \cite{Mohamadi}, while entropy and margin-based sampling strategies are also widely employed \cite{Roth2006}. Task-agnostic methods, such as Learn loss \cite{Yoo2019}, use a loss prediction module to estimate data points that are likely to be wrongly predicted. Among diversity-based strategies, Core-set \cite{Sener2017} is one of the most popular, using a K-center Greedy algorithm to locate a set of representative data points. Cluster-Margin \cite{Citovsky2021} combines uncertainty and diversity, while DRMRS \cite{Elhamifar2013} takes into account the margin and diversity. BADGE \cite{Ash2019} balances uncertainty and diversity using a $k-$\asc{MEANS++} seeding algorithm on gradients obtained from the last layer of the network. CDAL \cite{Agarwal2020} replaces the Euclidean distance with the pairwise contextual diversity in the greedy K-center algorithm used in the Core-set. CLUE \cite{Prabhu} performs uncertainty-weighted clustering to identify target instances that are uncertain according to the model and diverse in feature space. VAAL \cite{sinha2019variational} uses a Variational Autoencoder (VAE) to map instances into a latent space, which is then fed into a discriminator that learns to differentiate between labeled data and unlabeled samples.

\paragraph{\acl{AL} for Object Detection.} \acs{AL} approaches to object detection can be classified into black-box and white-box methods \cite{RoyUnmesh}. Black-box methods do not depend on the underlying network architecture and use informativeness scores, such as the confidence obtained from the softmax layer, while white-box methods are dependent on the architecture of the underlying network. The Minmax approach, which selects the least confident images among the unlabeled pool, is a popular black-box method \cite{RoyUnmesh}. Ensemble methods have also been used for object detection-oriented AL \cite{FengDi,Schmidt2020}. Query strategies based on localization tightness and stability \cite{Kao2018}, mixture density networks \cite{DBLP:journals/corr/abs-2103-16130}, and a unified box regression and classification metric \cite{WeipingYu} have also been proposed. MIAL \cite{Yuan2021} is a multiinstance framework that filters out noisy instances to bridge the gap between instance-level and image-level uncertainty. PPAL \cite{Yang2022} is a two-stage algorithm that includes difficulty-calibrated uncertainty sampling and category-conditioned matching similarity. \cite{Huang2022} proposed to cluster the unlabeled observations into groups based on the frequency domain values and to use different sampling rates for each group.

\subsection{Challenges of Stream-based Active Distillation} 
The importance of sampling has been first formulated in \cite{baykal2022robust} as the problem of developing KD methods that are both query-efficient and robust to labeling inaccuracies due to the imperfection of the teacher (i.e., \textit{confirmation bias}). Their methods provide a theoretical guarantee that the scheme leads to queries where the teacher provides the correct labels. However, this approach has been developed in a pool-based setting where the student has access to the entire information pool. In contrast, in stream-based scenarios, techniques such as diversity-based strategies, clustering, or pairwise distance matrices may not be feasible, especially in contexts where the spatio-temporal correlation among the data is significant. Another aspect is that, due to the complexity of the student model, uncertainty techniques relying on Monte Carlo dropout or Learn loss modules may not be viable options.

%adding complexity to the student model through ensembles,    and that it may not be necessary if we assume there are spatio-temporal correlation among the data that we could exploit.   

%Though, the method cannot be applicable in the SBAD scenario

%Although many state-of-the-art AL techniques have been proposed for pool-based settings, these methods may not , where each incoming image must be evaluated on the fly without storing a large number of previously seen images. In such cases,  Finally, the sampling strategies should take into account the imperfection of the teacher as an oracle. These challenges highlight the need for simpler and scalable active learning strategies that can facilitate the deployment of object detectors in stream-based systems. However, we propose that a more \textbf{robust} and \textbf{scalable} approach involves active learning. Assuming we are able to collect a sample of data from the target domain, a teacher is able to provide annotations from which the students can learn. This approach could help bridge the performance gap between large-scale models and affordable versions \cite{LucasBeyer2022}.


%\paragraph{Challenges of Stream-based Active Learning.} Although many state-of-the-art active learning techniques have been proposed for pool-based settings, these methods may not be applicable in scenarios where each incoming image must be evaluated on the fly without storing a large number of previously seen images. In such cases, techniques that rely on diversity-based strategies, such as clustering or pairwise distance matrices, may not be feasible. Additionally, given the limited storage capabilities of devices, adding complexity to the student model through ensembles, Monte Carlo dropout, or Learn loss modules may not be a viable option. These challenges highlight the need for simpler and scalable active learning strategies that can facilitate the deployment of object detectors in stream-based systems.

 

%If we need to select the most informative frames in a single-pass manner, where each incoming image needs to be evaluated on the fly, the state-of-the-art strategies proposed for pool-based AL cannot be implemented. Indeed, without storing a reasonable amount of images (or their embeddings) it is not possible to use diversity-based techniques based on clustering or pairwise distance matrices. Similarly, given the computational constraint imposed by the limited storage capabilities of the devices, adding complexity to the student model through the use of ensembles, MC dropout, or Learn loss modules is not a viable option. These premises highlight the need to consider simpler and scalable strategies that can facilitate the deployment of object detectors in stream-based systems. 


==> 4_SOTA/archives/ActiveLearning.tex <==



\subsection{Active learning}
\label{sec:SOTAActiveLearning}
%The selection of data for further labelling is under the scope of \textbf{Active Learning} (AL). In the \emph{pool-based} approaches, one assume a full access to all candidate data at selection time. However, in many real-world applications, a large number of unlabeled samples arrive in a stream, making it impossible to store all the data in a candidate-pool. Instead, a stream-based approach as \textit{single-pass} online learning is more suitable. In this approach, for each new incoming sample, it is decided in a one-shot experience whether it should be used for updating the model. 
%The research in \emph{active learning} cannot be transposed. Indeed,  KD is confronted to \textit{Confirmation bias} due to the imperfection of the teacher. The phenomenon refers to the noise accumulation when the model is trained using incorrect predictions for semi-supervised or unsupervised learning \cite{arazo2020pseudo}. Otherwise, commonly adopted methods \textbf{uncertainty-based} cannot be straightforwardly used.  
%The importance of sampling has been first formulated in \cite{baykal2022robust} as the problem of developing KD methods that are both query-efficient and robust to labelling inaccuracies. Their development was in a pool-based setting. Yet, in many real-world applications, a large number of unlabeled samples arrive in a streaming manner, making it impossible to maintain all the data in a candidate pool.
% \begin{itemize}
%     \item \cite{liu2021online} addresses the \emph{concept drift}, \emph{noise} and \emph{unlabeled data} in classification of data streams. Their selection strategy involves the estimation of a local density which is basically means that for an instance $x_i$, the number of times it is close to another instance (using Euclidian distance). The replacement policy is based the \emph{forgetting curve} \url{https://en.wikipedia.org/wiki/Forgetting_curve}. \textcolor{blue}{First, they study a classification problem and their selection strategy is yet to be proven on a detection task. Next, their replacement strategy focuses on an exponential law rather than a measure based on information theory metrics. We must implement this law and compare it}.  
% \end{itemize}

In a KD scheme, the development of specialized student models requires the generation of many pseudo-labels from a teacher model, which can be an expensive and time-consuming task. As the teacher is generally represented by a large and complex model, making a prediction for each incoming frame can be computationally expensive. Moreover, if the teacher model is running on a cloud-based platform, there may be monetary costs associated with using the platform, such as hourly usage fees or data transfer costs. This highlights the necessity to select a smaller yet informative subset of the data to be pseudo-labeled. To this end, active learning (AL) can be highly beneficial as it enables an efficient model development by smartly selecting the most useful observations, according to a pre-defined instance selection criterion. Unfortunately, the majority of active learning strategies proposed in the literature assume dealing with a perfect oracle, while in KD the teacher model might not always provide a correct label. This can create a phenomenon of confirmation bias, where the noisy or incorrect labels provided by the teacher might degrade the predictive performance of the student models \cite{arazo2020pseudo,LiuTan}. In particular, Baykal et al. \cite{Baykal2022} highlighted how the use of margin-based active learning (AL) can exacerbate the issue of confirmation bias in KD, despite being one of the most widely employed query strategies \cite{TongKoller}. Margin-based AL is an uncertainty-based sampling scheme used in classification, where the most informative data points are deemed to be the ones lying close to the decision boundary \cite{Balcan,Roth}. In general, uncertainty-based sampling strategies try to focus on data points that the model is least confident about, in order to reduce its uncertainty. Other types of sampling strategies include disagreement-based AL \cite{Hanneke2014,Seung1992,Freund1997}, diversity and density-based methods \cite{Ge2014,preclustering,Zhang2020}, expected error or variance minimization \cite{err1,err2}, and expected model change maximization \cite{Cai2013}. Finally, hybrid strategies can be used by combining multiple instance selection criteria \cite{Donmez2007,Huang2014}. In computer vision, the majority of the currently proposed approaches can be grouped into two categories: uncertainty-based and diversity-based strategies.

With regard to the way the student models interact with the unlabeled instances, we can identify three macro AL scenarios, as outlined in \cite{Settles2009}. The first scenario is pool-based AL, which is an offline setting where a dataset is partitioned into a labeled and an unlabeled set. This scenario is the most widely studied in the literature and it is suitable when the unlabeled set is large and can be accessed multiple times by the learner. The second scenario is stream-based AL, where data is coming in a continuous stream and the learner must decide on the fly which examples to request labels for. The third scenario is membership query synthesis, where the learning algorithm can decide which examples to generate to maximize the information gained about the underlying data distribution. This scenario is appropriate when the data is scarce or expensive to obtain and generating new data is relatively inexpensive.

\subsubsection{Pool-based active learning.}
In pool-based AL, we assume the availability of a large set of unlabeled instances $\mathcal{U}$, from which we need to select a subset of informative instances to be labeled and used to train our model. In Figure \ref{fig:al_pool_based}, we can see a flowchart representing a possible KD pipeline implemented with a pool-based approach. Specifically, we first collect $N$ unlabeled observations and form a candidate pool of instances. Next, we employ an instance selection criterion to select the most informative instances from the pool, according to the labeling budget constraint $b$. These instances are then pseudo-labeled by the teacher model and incorporated into the training set to fine-tune the specialized student model. It should be noted that the pipeline outlined follows a batch mode AL approach, where the model is updated only when a set of labeled examples have been gathered. This method is widely used when dealing with complex deep neural networks as it is computationally more efficient than the alternative one-by-one sampling strategy, which updates the model each time a new label is received \cite{Ren2022,Elhamifar2013}.

In computer vision, despite a recent spark of interest in object detection, active learning has been mostly studied for image classification tasks.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=\linewidth]{0_images/AL_pool_based.png}
    \caption{KD through pool-based AL.}
    \label{fig:al_pool_based}
\end{figure}

\paragraph{Image classification.} 
Uncertainty-based sampling strategies are among the most employed ones in image classification tasks. Among these, entropy \cite{Shannon1948} is one of the most common instance selection criteria, as it provides a measure of the uncertainty of a random variable. In a setting with $k$ classes, the model uncertainty can be measured using the entropy of the predicted class probabilities as in
$$entropy(x) = -\sum_{i=1}^{k} p(y = c_i|x)log p(y = c_i|x)$$
Instances are selected for annotation by choosing those with the highest entropy, indicating the model is the least certain of their class. However, as highlighted by Joshi et al. \cite{5206627}, although entropy is a good indicator of the uncertainty of the prediction, it might not be the best measure when a large number of classes are present in the data. Indeed, small probability values associated with unimportant classes may contribute to a high entropy score even for samples that are not significantly uncertain. To overcome this issue, margin-based sampling only considers the difference between the largest two predicted class posterior probabilities \cite{5206627,Roth2006} as in
$$margin(x) = p(y = c_b|x)-p(y = c_{sb}|x)$$
where $c_b$ and $c_{sb}$ are the classes with highest predicted probabilities. According to this strategy, the instances with the lowest margin are deemed to be the most informative ones. Another approach to uncertainty estimation in deep models is represented by Monte Carlo (MC) dropout \cite{Gal2017}. MC dropout is a Bayesian approximation method that consists in applying a dropout layer before each weight layer of the network. At test time, in order to sample from the approximate posterior, $T$ stochastic forward passes are performed with dropout applied. Subsequently, an estimate of the prediction uncertainty for a given class $c$ is obtained by marginalizing over the approximate posterior using MC integration:
\begin{equation*}
    \begin{aligned}
    p(y=c|x) & = \int p(y=c|x, w)p(w|\mathcal{D}_{train})dw
    \\ & \approx \int p(y=c|x, w)q_{\theta}^*dw
    \\ & \approx \frac{1}{T}\sum_{t=1}^{T}p(y=c|x, \hat{w}_t)
    \end{aligned}
\end{equation*}
where $p(w|\mathcal{D}_{train})$ is the true model posterior distribution of the network weights $w$ given a training set $\mathcal{D}_{train}$, and $\hat{w}_t \sim q_{\theta}^*$ given the dropout distribution $q_{\theta}$. An alternative to MC dropout is the use of ensembles \cite{Mohamadi}. In this case, an uncertainty estimate can be obtained by averaging the predictions obtained with $K$ networks trained on the same data
$$p(y=c|x)=\frac{1}{K}\sum_{i=1}^{K}p(y=c|x, w_i)$$
where $w_i$ are different random weight initializations. Besides targeting uncertain data points, another common strategy is to identify a representative subset of the data. One significant method pursuing this objective is core-set \cite{Sener2017}, which uses a k-centre-Greedy algorithm to locate a set of representative data points. The objective function is given by
$$\min_{s^1:|s^1|\leq b} \max_i \min_{j \in s^1 \cup s^0} \Delta(x_i, x_j)$$
where $s^1$ is the set of points to be queried, $s^0$ is the initial labelled set, and $\Delta(\cdot, \cdot)$ is the distance measure obtained using the $l_2$ distance between the activations of the final fully-connected layer. The solution to this objective function is found using a 2-approximation algorithm. The key idea is to select $b$ data points such that the largest distance between a data point and its nearest center is minimized. Batch active learning by diverse gradient embeddings (BADGE) \cite{Ash2019} represents another strategy to exploit the last layer of the network. This approach strikes a balance between uncertainty and diversity using a $k-$ \asc{MEANS++} seeding algorithm on the gradients obtained from the last layer of the network, with respect to the predicted label. The gradients are used as a proxy for the model uncertainty on the unlabeled instance. Intuitively, the gradient embedding for a data point will have a large norm if the model is uncertain about its label. Cluster-margin \cite{Citovsky2021} represents another active learning approach that tries to combine uncertainty and diversity. It does this by leveraging hierarchical agglomerative clustering and then selecting the samples with the lowest margin from each cluster. More specifically, clusters are estimated from the embedding obtained from the penultimate layer of the network. Then, in trying to balance the trade-off between uncertainty and diversity, the instances with the lowest margin scores are drawn from each cluster according to a round-robin scheme. A hybrid strategy based on margin sampling has also been used by Elhamifar et al. \cite{Elhamifar2013}, who leveraged a dissimilarity-based sparse representative selection (DSMRS) algorithm \cite{10.5555/2999134.2999137,7364258}. The uncertainty module takes into account the margin, while the diversity aspect is evaluated with a dissimilarity matrix that is computed to represent the pairwise dissimilarities between the unlabeled data points. Two other important strategies that combine instance uncertainty with the diversity criterion are the contextual diversity for active learning (CDAL) \cite{Agarwal2020} approach and the clustering uncertainty-weighted embeddings (CLUE) method \cite{Prabhu}. The CDAL approach has been developed in two variants. The first framework is referred to as CDAL-CS, and it leverages the K-center-Greedy algorithm used in core-set \cite{Sener2017}, replacing the Euclidean distance with the pairwise contextual diversity. This statistic reflects the model uncertainty by computing the KL divergence between the predicted probability vectors. The second framework, CDAL-RL, undertakes a reinforcement learning approach using contextual diversity as part of a Bi-LSTM-based policy. The policy network receives in input the image representation obtained from the task network, and the labeling decision is modeled as a Bernoulli random variable using the sigmoid activation at the output of the Bi-LSTM network. The reward function takes into account contextual diversity, visual representation, and semantic representation. Finally, CLUE performs uncertainty-weighted clustering to identify target instances for labeling that are both uncertain according to the model and diverse in feature space. Sinha et al. \cite{sinha2019variational} proposed a diversity-based approach that uses a VAE to map the instances into a latent space, which is then fed into a discriminator that learns to differentiate between the labeled data already available and the unlabeled samples. This approach is referred to as variational adversarial active learning (VAAL). A different take on active learning has been suggested by Yoo and Kweon \cite{Yoo2019}, who proposed the learning loss for active learning (LLAL) strategy. This is a task-agnostic method that augments the model by introducing a loss prediction module, which is used to estimate the data points for which the task network is likely to produce a wrong prediction.

\paragraph{Object detection.}
Conversely to the image classification case, very few works focused on the development of active learning strategies for object detection tasks. Liu et al. \cite{Liu2015} proposed using maximum mean discrepancy (MMD) as a statistical test in active learning for object detection. The method involves measuring the difference between the probability distributions of two sets of data, namely the distribution of object proposals generated by an object proposal algorithm and the distribution of object instances in the training set. By selecting object proposals with a high MMD score, which suggests that they are dissimilar to the instances already in the training set, the authors aim to enhance the diversity of the training set and improve object detection performance.

Roy et al. \cite{RoyUnmesh}  suggested a classification of active learning approaches for single-shot multi-box detectors into two categories. Black-box methods do not depend on the underlying network architecture,  but they use informativeness scores as the confidence obtained from the softmax layer. Instead, white-box methods are dependent on the architecture of the underlying network used to obtain the predictions. Among the black-box methods, the authors suggested using the minmax approach, which selects the least confident images among the unlabeled pool. According to this strategy, the confidence of an image is given by the maximum confidence score between the detected bounding boxes. The query function is given by
$$\argmin_i \max_c max_{j \in \{b_{ic}\}}prob(j)$$
where $\{b_{ic}\}$ are the bounding boxes found in the $i$th image , related to class $c$. In multi-class settings, the authors also consider the maximum entropy approach. With regard to the white-box methods, the authors proposed a query-by-committee method that uses a base network and a set of extra convolution layers to detect objects at different scales. Then, a disagreement measure is obtained by comparing the bounding boxes obtained from the base model and the additional layers. Similarly to the minmax strategy, Brust et al. \cite{Brust2018} evaluated the performance of the best-versus-second-best margin scores with different aggregation functions over all the bounding boxes detected in an image. The aggregation functions used are sum, average, and maximum. 


The tightness criterion estimates the certainty of the localization by measuring the intersection over union (IoU) between the region of interest (RoI) proposed at the beginning of the training and the bounding boxes obtained in the final output. Instead, the stability criterion is based on whether the detected bounding boxes are sensitive to changes in the input image. It is measured as the IoU between several instances of the same sample affected by different injected Gaussian noises. Feng et al. \cite{FengDi} proposed an active learning strategy for training a LiDAR 3D object detector based on MC dropout and deep ensembles. After estimating the predictive probability using those two methods, the authors used an entropy-based query function to select the most uncertain samples. Schmidt et al. \cite{Schmidt2020} further investigated ensemble-based active learning for 2D object detection ensemble networks.  Inspired by  \cite{Kao2018},  they introduced a consensus score metric based on localization uncertainty, which computes the IoU matrix by comparing the RoI proposals obtained by the committee members. They also considered a variation ratio-based variant of the consensus score, by taking into account the distribution of the detected classes and a temporal version of the RoI matching measure. The key intuition behind the sequence RoI matching is that sampling along consecutive time steps can be used as a proxy for multiple forward passes for the same image,  obtaining an estimate for the network uncertainty over a time horizon. However, the applicability of this approach can be limited by the specific FPS value used.  In trying to avoid the high computational costs related to uncertainty estimation via MC dropout or ensembles, Choi et al. \cite{DBLP:journals/corr/abs-2103-16130} proposed a strategy based on mixture density networks that estimates a probabilistic distribution for each localization and classification head's output.  Yu et al. \cite{WeipingYu}  proposed a consistency-based active learning strategy for object detection (CALD). Their algorithm unifies box regression and classification within a single metric, and takes into account the consustency between the original and augmented images. Finally, to alleviate unbalanced class distribution, they monitor the distance of the class distribution of the sampled images from the one of the labeled pool. Yuan et al. \cite{Yuan2021} proposed a multiple-instance framework to bridge the gap between the instance-level and image-level uncertainty by filtering out noisy instances. They first highlight informative instances within the unlabeled set and highlight its distribution to the labeled set. Then, the uncertainty of a single image is estimated by re-weighting the uncertainty of the individual instances. A possible issue of this approach is ignoring the instance-level redundancy, which can be defined as instances with similar appearances presented in the same context. To tackle this issue, Wu et al. \cite{WuEntropy} combined uncertainty  and diversity using a two-stage procedure. Initially, the uncertainty of each image is estimated by computing the entropy on the feature space. Successively,  they focus on intra-class and inter-class diversity by using class-specific prototypes.  Another strategy that combines uncertainty-based and diversity-based sampling has been proposed by Yang et al. \cite{Yang2022}. They proposed a plug-and-play active learning (PPAL) algorithm composed of two modules, difficulty-calibrated uncertainty sampling and category-conditioned matching similarity, where the similarity is measured using the L2 similarity of averaged convolutional feature maps. Aghdam et al. \cite{Aghdam2019} proposed a new function to score the importance of each pixel for improving the detector.  An image-level metric is then obtained by aggregating the pixel-level scores. Huang et al. \cite{Huang2022} proposed a method for selecting images based on their frequency domain values, which are calculated using a Fourier Transform. This is because deep neural networks are more sensitive to edges, which correspond to high frequencies. First, the low frequency components are removed, and the image is restored using an inverse Fourier Transform. Then, the image is divided into regions, and the one with the largest frequency values is removed to select images with more scattered edge information. The sum of frequency values is calculated, and the images are divided into groups for sampling. Finally, similar images are removed based on cosine similarity of weighting frequency domains to increase diversity.

\subsubsection{Stream-based active learning.}
The application of pool-based AL strategies requires storing a large number of unlabeled instances in a candidate pool, from which the learner can then select the top $k$ data points to be labeled. While this approach facilitates the selection of the most informative examples, it cannot be easily applied in many real-world scenarios, where samples arrive at a high frequency in the form of a data stream. Moreover, small edge devices like CCTV cameras or other affordable hardware often have limited internal storage, which makes it difficult to store a large number of frames before deciding which ones should be labeled. That is why it would be beneficial to guide the data collection scheme using a stream-based AL approach. An overview of active learning strategies for dealing with data streams has been proposed in \cite{surveyOAL}. While there have been some online active learning approaches for image classification using traditional statistical models \cite{ROZANEC2022277,Narr2016}, the use of deep learning models for object detection coupled with stream-based active learning has never been investigated.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=\linewidth]{0_images/AL_stream_based.png}
    \caption{KD through stream-based AL.}
    \label{fig:al_pool_based}
\end{figure}


\subsection{Sampling strategies}

\subsubsection{Pool-based}
These strategies assume the availability of a candidate set of unlabeled frames, from which an informative subset needs to be identified. Despite this scenario being the most commonly studied one in the active learning literature, we used it as a playground to observe the behavior of simple strategies that can be easily adapted to a stream-based setting for knowledge distillation.

\begin{itemize}
    \item Random: $N$ frames are sampled at random from the candidate pool.
    \item Least confidence: the most informative observations are deemed to be the ones with the smallest confidence scores. As the object detector outputs a confidence score for each instance in the image, we tested this strategy with two different aggregation functions:
    \begin{itemize}
        \item[-] Min: this aggregation function estimates the confidence of an image with the confidence of the most uncertain object identified. This aggregation favors the presence of an uncertain object but does not deny the presence of other objects with a larger confidence score associated.
        \item[-] Max: this aggregation function estimates the confidence of a frame using the most confident object. Minimizing the max confidence is equivalent to seeking images mostly composed of a single, uncertain object.
    \end{itemize}
    \item Top confidence: in trying to fight the confirmation bias, this strategy tries to select frames for which the teacher is likely to provide correct pseudo labels. Aggregating by summation, we are furthermore seeking frames where many (confident) objects are present.
    \item Frequency: 
    \item N first: this strategy represents a na\"ive approach where the first observed frames are sent to the teacher.
\end{itemize}

\subsubsection{Stream-based}
In this case, we assume to be in a zero-storage scenario, where a candidate set of unlabeled frames is not available to the learner and a decision about sampling must be made on the fly.
\begin{itemize}
    \item Uniform: given a sampling rate $\alpha$, which represents the ratio of frames we are willing to pseudo label out of the incoming data stream,  we decide whether or not to sample a frame by iteratively drawing a uniform random variable. At each time step $t$, we draw a number $s \sim U(0,1)$, and we only sample the frame when $s \geq (1-\alpha)$.
    \item Least confidence with Bernoulli: at each time step $t$,  we draw a number from a Bernoulli random variable of parameter $b/(b+c)$, where $c$ is the confidence of the frame and $b>0$ is a smoothing parameter used to adjust the sampling rate. For confidence scores approaching zero, the sampling probability converges to 1.
    \item Top confidence with thresholding: this strategy works by selecting observations whose confidence score exceeds a given threshold. In this case, the threshold is estimated using a warm-up phase, where frames are observed for a while without sampling in order to obtain a $(1-\alpha)$-upper percentile to be used to seek confident frames. This strategy is still feasible in a stream-based manner as the warm-up phase only requires storing a single scalar for each image.
\end{itemize}








==> 4_SOTA/archives/KD_sota_cvpr.tex <==
\subsection{Knowledge Distillation}
KD is a research area often characterized by the \emph{teacher-student} framework \cite{wang2021knowledge}. A teacher 
model aims at distilling knowledge during the training phase of a 
student model. A KD process can have two purposes: Unsupervised Domain 
Adaptation (UDA) \cite{oza2021unsupervised} and Model Compression (MC).

\paragraph{Unsupervised Domain Adaptation. } UDA aims at preventing the performance loss of a model when it infers on a dataset distributed differently than the source domain. For example in \cite{soviany2021curriculum}, researchers argue there is no dataset large enough to cover all aspects of an urban city scenario, and therefore a general-purpose detector may produce poor performance on the target domain if the model is not adapted. To cope with this decrease in quality, \cite{khodabandeh2019robust,li2021free,inoue2018cross} focus on incrementally enhancing the performance of an object detector over the target domain by considering the model's predictions as noisy and iteratively eliminating false positives and false negatives. Alternatively, \cite{xu2019self}'s approach enables the model to learn domain-invariant features for semantic segmentation through an attention mechanism. The student focuses thus on the discriminant features that are not modified according to the context. Other approaches as in \cite{kang2017noscope}, propose to take an image in the target domain that will be set as the reference in a two-stage processing scheme. The latter involves a first stage using a \emph{difference detector} to extract the vehicles, followed by a \emph{classification} performed by the student. The teacher model supervises both the difference detector and the classifier. The last discussed approach is presented in \cite{mhalla2016faster}. It consists of the specialization of a generic detector (e.g., Faster R-CNN), using a sequential Monte Carlo filter to adapt the detector to an unlabeled target video sequence. The training set generation is supported by the filter which considers the teacher predictions as samples from an unknown distribution. The false positives and false negatives are gradually eliminated by defining a likelihood function that allows converging to more accurate teacher predictions. 

\paragraph{Model Compression. } These applications aim at producing lightweight models more  suitable to the storage and computational capacities of a miniaturized device. The challenge is to bring the student to perform as well as the teacher and larger model. The difficulty is that the smaller network may find it challenging to construct the features map as discriminating as the teacher network \cite{rivas2022towards}. This difficulty/risk could be mitigated under the assumption that a camera in a static surveillance network observes a particular context within the ensemble of contexts existing in a city \cite{bhardwaj2022ekya}. Otherwise, there may only need to model the distribution of that specific context. This assumption has been a basis for the work of \cite{shen2017fast}. The authors propose to skew the class distribution of a large dataset by considering short-term distributions, which can be processed by simpler models due to the small number of classes. To this end, they implement a model selection policy by minimizing the processing time while maintaining the accuracy above a given threshold. This approach requires only one offline training. Under the same assumption, \cite{cai2019once} uses the pruning on a general-purpose deep neural network to generate shallower models. The benefit is the reduction of training costs as no retraining is needed, yet the domain shift issues are not mentioned in the work.

\paragraph{Online Distillation. }In \cite{cioppa2019arthus} the authors designed an online knowledge distillation scheme to perform real-time human segmentation in sports videos.  The 
student performs the inference in real-time while its weights are often updated by an offline student-teacher framework. Experiments show the model's ability to adapt to variations occurring in the context. It even outperformed in some cases the teacher.  Online distillation is also employed in \cite{mullapudi2019online} to adapt a low-cost semantic segmentation model to a target video where the data distribution is not necessarily stationary. The student model appears to exhibit better temporal stability than the teacher model. 

\paragraph{Context-aware distillation. } The latest research suggests that the use of prior knowledge about a scene and broadly speaking its contextual features could lead to inexpensive and more specialized students \cite{rivas2022towards}. While the paper does not specify which features, we claim that their position constitutes an interesting research direction. As an example, \cite{delta_distillation_2022}, suggests that adding a temporal dimension benefits knowledge distillation. In their proposal, the student learns the variations in the teacher’s
intermediate features over time. They demonstrate thus that these temporal variations can be effectively distilled due to the temporal redundancies within video frames. An alternative way of looking at the problem is that not every frame is relevant for learning. To the best of our knowledge, there is no work that analyzes how frequently and when should we integrate a frame in the training pipeline.

==> 4_SOTA/archives/KD_sota_cvpr_short.tex <==
%KD is a research area that utilizes a \emph{teacher-student} framework \cite{wang2021knowledge}. The teacher model distills knowledge during the training phase of a student model, and the KD process can have two purposes: Unsupervised Domain Adaptation (UDA) and Model Compression (MC). Also, we can identify two main KD approaches: online distillation and context-aware distillation.
%\paragraph{Unsupervised Domain Adaptation. } UDA aims to prevent the performance loss of a model when it infers on a dataset distributed differently than the source domain. Approaches such as \cite{khodabandeh2019robust,li2021free,inoue2018cross} focus on incrementally enhancing the performance of an object detector over the target domain by iteratively eliminating false positives and false negatives. Alternatively, \cite{xu2019self} enables the model to learn domain-invariant features for semantic segmentation through an attention mechanism. Other approaches, such as \cite{kang2017noscope}, propose a two-stage processing scheme using a \emph{difference detector} and a student classifier supervised by the teacher model. In \cite{mhalla2016faster}, a generic detector is specialized using a sequential Monte Carlo filter to adapt the detector to an unlabeled target video sequence.
%\paragraph{Model Compression. } These applications aim to produce lightweight models that are more suitable for the storage and computational capacities of miniaturized devices. The challenge is to bring the student to perform as well as the teacher and larger model. \cite{shen2017fast} proposes to skew the class distribution of a large dataset by considering short-term distributions, which can be processed by simpler models due to the small number of classes. \cite{cai2019once} uses pruning on a general-purpose deep neural network to generate shallower models.
%KD is a research area that leverages a teacher-student framework \cite{wang2021knowledge}. The teacher model transfers knowledge to a student model during training, with two main purposes: Unsupervised Domain Adaptation (UDA) and Model Compression (MC). UDA aims to prevent the performance degradation of a model when it operates on a dataset that has a different distribution than the source domain. Various approaches such as \cite{khodabandeh2019robust,li2021free,inoue2018cross} incrementally improve the performance of an object detector in the target domain by iteratively reducing false positives and negatives. Alternatively, \cite{xu2019self} learns domain-invariant features for semantic segmentation through an attention mechanism. Other approaches, such as \cite{kang2017noscope}, propose a two-stage processing scheme using a difference detector and a student classifier supervised by the teacher model. On the other hand, MC aims to generate lightweight models that are more suitable for miniaturized devices. The main challenge is to maintain the student's performance while reducing its complexity. \cite{shen2017fast} proposes to skew the class distribution of a large dataset by considering short-term distributions, which can be processed by simpler models due to the small number of classes. \cite{cai2019once} uses pruning on a general-purpose deep neural network to generate shallower models. Two main KD approaches are online distillation and context-aware distillation.

\subsection{Knowledge Distillation}


\ac{KD} is a method that involves training a smaller model to imitate the performance of a larger model. The main objectives of this technique are to prevent a decrease in the model's performance when it operates on a data set that is distributed differently than the source domain, referred to as Unsupervised Domain Adaptation (UDA), and to produce lightweight models suitable for the storage and computational capacities of miniaturized devices, referred to as Model Compression (MC) applications. In this study, we use a technique called \emph{Self-training with knowledge distillation}, which was introduced by \cite{originSelfDistillaion}. This technique trains a student model using pseudo-labels generated by a teacher model, which is beneficial when the labeled data is limited but we have access to a large sample of unlabeled data. Furthermore, the aforementioned distillation scheme does not need a direct access to the teacher. Yet, it may also propagate errors or biases. 

In addition, we will discuss two additional techniques of interest in the following paragraphs: online distillation and context-aware distillation. 

\paragraph{Online Distillation.} This approach involves training a smaller student model to mimic the output of a larger teacher model on a per-example basis. In \cite{cioppa2019arthus}, the authors designed an online knowledge distillation scheme to perform real-time human segmentation in sports videos. Experiments show the ability of the model to adapt to contextual variations. Online distillation is also employed in \cite{mullapudi2019online} to adapt a low-cost semantic segmentation model to a target video where the data distribution is not necessarily stationary.

\paragraph{Context-aware Distillation.} The works in \cite{rivas2022towards,delta_distillation_2022} attempt to exploit the contextual characteristics of the scene to develop effective \ac{KD}. They directly worked on the distillation scheme to develop more specialized students. For example, \cite{delta_distillation_2022} added a temporal dimension such that the student learns the variations in the intermediate features of the teacher over time, taking into account the redundancies of the frames within a CCTV stream. 


% is a research area that involves a teacher-student framework \cite{wang2021knowledge}, which involves the teacher model distilling knowledge to a student model during training. \ac{KD} can serve two purposes: , which aims to prevent performance loss when inferring on a different dataset, and \acf{MC}, which produces lightweight models for smaller devices. For \ac{UDA}, there are several approaches like \cite{khodabandeh2019robust,li2021free,inoue2018cross} that enhance object detection, while \cite{xu2019self} learns domain-invariant features using an attention mechanism. \ac{MC} applications include \cite{shen2017fast}, which skews the class distribution to process smaller classes with simpler models, and \cite{cai2019once}, which prunes a \acl{DNN} to produce shallower models.

==> 4_SOTA/archives/KnowledgeDistillation.tex <==
\subsection{Knowledge distillation}
\label{sec:sotaKD}
Knowledge Distillation (KD) is a research area often characterized by the \emph{teacher-student} framework \cite{wang2021knowledge}. A teacher 
model aims at distilling its knowledge during the training phase of a 
student model. A KD process can have two purposes: Unsupervised Domain 
Adaptation (UDA) \cite{oza2021unsupervised} and Model Compression (MC).\\
\subsubsection{Unsupervised Domain Adaptation}
UDA aims at preventing the performance's loss of a model when it infers on a dataset distributed differently than the source domain. For example in \cite{soviany2021curriculum}, researchers argue there is no dataset large enough to cover all aspects of an urban city scenario, and therefore a general-purpose detector may produce poor performance on the target domain if the model is not adapted. To cope with this decrease in quality, \cite{khodabandeh2019robust,li2021free,inoue2018cross} focus on incrementally enhancing the performance of an object detector over the target domain by considering the model's predictions as noisy and iteratively eliminating false positives and false negatives. Alternatively, \cite{xu2019self}'s approach enables the model to learn domain-invariant features for semantic segmentation through an attention mechanism. The student focuses thus on the discriminant features that are not modified according to the context. Other approaches as in \cite{kang2017noscope}, propose to take an image in the target domain that will be set as the reference in a two-stage processing scheme. The latter involves a first stage using a \emph{difference detector} to extract the vehicles, following by a \emph{classification} performed by the student. The teacher models supervises both the difference detector and the classifier. The last discussed approach is presented in \cite{mhalla2016faster}. It consists in the specialization of a generic detector (e.g., Faster R-CNN), using a sequential Monte Carlo filter to adapt the detector to an unlabeled target video sequence. The training set generation is supported by the filter which considers the teacher predictions as samples from an unknown distribution. The false positives and false negatives are gradually eliminated by defining a likelihood function which allows to converge to more accurate teacher predictions. 

\subsubsection{Model compression}applications aims at producing lightweight models more  suitable to the storage and computational capacities of a miniaturized device. The challenge is to bring the student performs as well as the teacher and larger model. The difficulty is that the smaller network may find it challenging to construct the features map as discriminating as the teacher network \cite{rivas2022towards}. This difficulty/risk could be mitigated under the assumption that a camera in a static surveillance network observes a particular context within the ensemble of contexts existing in a city \cite{bhardwaj2022ekya}. Otherwise, there may only need to model the distribution of that specific context. This assumption has been a basis for the work of \cite{shen2017fast}. The authors propose to skew the class distribution of large dataset by considering short-term distributions, which can be processed by simpler models due to the small number of classes. To this end, they implement a model selection policy by minimizing the processing time while maintaining the accuracy above a given threshold. This approach requires only one offline training. Under the same assumption, \cite{cai2019once} uses the pruning on a general-purpose deep neural network to generate shallower models. The benefit is the reduction of training cost as no retraining is needed, yet the domain shift issues are not mentioned in the work.
\subsubsection{Online Distillation}is also possible. In \cite{cioppa2019arthus} the authors designed an online knowledge distillation scheme to perform real-time human segmentation in sports videos.  The 
student performs the inference in real time while its weights are often updated by an offline student-teacher framework. Experiments show the model's ability to adapt to variations occurring in the context. It even outperformed in some cases the teacher.  Online distillation is also employed in \cite{mullapudi2019online} to adapt a low-cost semantic segmentation model to a target video where the data distribution is not necessarily stationary. The student model appears to exhibit better temporal stability than the teacher model. 
\subsubsection{Context-aware distillation.}
The latest research suggests that the use of prior knowledge about a scene and broadly speaking its contextual features could lead to inexpensive and more specialized students \cite{rivas2022towards}. While the paper does not specify which features, we claim that their position constitute an interesting research direction. As an example, \cite{delta_distillation_2022}, suggests that adding a temporal dimension benefits the knowledge distillation. In their proposal, the student learns the variations in the teacher’s
intermediate features over time. They demonstrate thus that these temporal variations can be effectively distilled due to the temporal redundancies within video frames. An alternative way of looking at the problem is that not every frame is relevant for learning. At the best of our knowledge, there is no work that analyzes how frequent and when should we integrate a frame in the training pipeline.



%use the foundation of teacher-student to produce models light enough to be stored and run in real-time in embedded devices. One of the main problems with model compression is the severe limitation of the shallow model, the student, to perform as well as the teacher's model on the same dataset. This may be due to the fact that the student's network has difficulty constructing feature maps that are as discriminating as the teacher network to cope with the intricacies of the data distribution \cite{rivas2022towards}. 



==> 4_SOTA/archives/SOTA_FULL.tex <==
\subsubsection{Knowledge distillation}
\begin{itemize}
    \item \textit{Knowledge distillation and student-teacher learning for visual intelligence: A review and new outlooks}\cite{wang2021knowledge} : This is a major survey. Many of the following papers are cited in this survey. 
    \item \textit{Arthus: Adaptive real-time human segmentation in sports through online distillation}\cite{cioppa2019arthus} : The authors design a online knowledge distillation scheme in order to perform real-time human segmentation in sport videos. Instead of using a time-consuming model, a light-weight model is progressively trained on live video sequence thanks to a teacher model. The student model performs inference in real-time while its weights are sometimes updated by a offline student-teacher framework. The experiments show the capacity of the model to adapt itself to context variations, but also seems to eventually outperforms its teacher by providing better results. 
    \item \textit{Noscope: optimizing neural network queries over video at scale}\cite{kang2017noscope} : The paper presents a system for querying videos for reducing the cost of neural network analysis via inference-optimized model search. That is, a difference detector helps to extract frame of vehicles in a video and then a student neural network is responsible to classify the content of the frame. A heavy teacher network provides supervision to both the difference detector and the classifier. This approach allows the model to adapt to a short-term video sequence while being suited for real-time applications.
    \item \textit{Self-ensembling attention networks: Addressing domain shift for semantic segmentation}\cite{xu2019self} : The authors build self-ensembling attention networks to reduce the domain gap between different datasets, the teacher and student networks has the same architecture since this work does not focus on model compression. Their approach allows the models to learn domain-invariant features for semantic segmentation thanks to an attention mechanism that forces the student network to focus on salient elements. However, the performance of the student segmentation depends too much on the teacher annotation quality.
    \item \textit{Online model distillation for efficient video inference}\cite{mullapudi2019online} : In this paper, the model distillation technique is employed to specialize accurate and low-cost semantic segmentation models to a target video steam. The student model is trained in an online fashion in order to be adapted for real-time scenario where the target video is not necessarily stationary. The model also seems to exhibit better temporal stability than it's teacher. 
    
\end{itemize}


\subsubsection{Models specialization}
\begin{itemize}
    \item \textit{Train one network and specialize it for efficient deployment}\cite{cai2019once} : they address the problem of inference across several edge devices by a once-for-all network training. It consists of training a general-purpose network before generating smaller networks (via network pruning) which could be deployed in specific hardware configuration without retraining. Their approach is effective for reducing the training cost of large scale deployment and to address the hardware constraints by including the targeted architecture in the loop. However, their once-for-all network is trained on ImageNet while the sub-networks are tested on this same dataset. Therefore, this paper is mainly about model compression without data context modification.
    \item \textit{Faster R-CNN scene specialization with a sequential Monte-Carlo framework}\cite{mhalla2016faster} : The authors highlight the decrease in precision when a deep neural network is tested on a dataset with large variations compared to the training set. To solve this issue, they propose to specialize generic detectors such as Faster R-CNN by utilizing a sequential Monte Carlo filter to adapt the detector to a unlabeled target video sequence. The training set generation is supported by the Monte-Carlo filter which considers the detections of the current model as samples from an unknown distribution. The false-negative and false-positive samples are progressively removed thanks to the definition of a likelihood function, however the moving objects are prioritized in the sample selection which could be an inconvenient for still objects, such as parked vehicles.
    \item \textit{Fast video classification via adaptive cascading of deep models}\cite{shen2017fast} : The authors proposes to skew the class distribution of a large dataset by considering short-term distributions, which can be processed by simpler models due to the fact that the number of visible classes is small. To this end, they develop a model selection policy by selecting several models among a collection by minimizing the processing time while maintaining the accuracy over a given threshold. Their solution speeds up face recognition on TV episodes and movies with little loss in accuracy compared to a modern CNN.  
\end{itemize}


\subsubsection{Unsupervised Domain Adaptation}
\begin{itemize}
    \item \textit{Unsupervised domain adaptation of object detectors: A survey}\cite{oza2021unsupervised} : This is a major survey. Many of the following papers are cited in this survey.
    
    \item \textit{Curriculum self-paced learning for cross-domain object detection}\cite{soviany2021curriculum} : The papers addresses the problem of domain adaptation with unlabeled target domain. The approach combines Cycle-GAN transformations and self-paced learning algorithm that lean from easy to hard. In practice, a metric helps to quantify the \textit{difficulty} of detecting the objects within an image. The network is first trained on easy samples and keep growing in detection difficulty which allows to increase the precision. 
    
    \item[S] \textit{A robust learning approach to domain adaptive object detection}\cite{khodabandeh2019robust} : In this paper, the authors proposes a a robust object detection framework which is resilient to noise in bounding box class labels. This approach allows to handle the domain shift for unsupervised domain adaptation for self-driving car context. Their method continuously correct the false positive and negative through the iterations and integrates other sources of information using a detection re-scoring function.
    
    \item[B] \textit{Cross-domain weakly-supervised object detection through progressive domain adaptation}\cite{inoue2018cross} : 
    
    \item[A] \textit{A free lunch for unsupervised domain adaptive object detection without source data}\cite{li2021free} : The paper highlights the problem of data privacy and thus proposes to perform an unsupervised domain adaptation without the source data. To this end, a self-entropy descent metric is build to quantify the quality of the generated pseudo labels. The authors observe the dominance of false negative samples in the pseudo labels and attempt to correct this issue with false negative mining. Their approach achieves good performances but false negative are still present and the authors point out the difficulty to completely remove them in a unsupervised way. 
    
\end{itemize}

\subsubsection{Large scale deployment}
\begin{itemize}
    \item[A] \textit{Towards automatic model specialization for edge video analytics}\cite{rivas2022towards} : The paper handles the difficulty of obtaining state-of-the-art accuracy while having limited access to computational resources in the context of real-time edge analytics. The authors highlight the potential benefits of having cameras which are observing a very specific and limited context and thus propose to train a context-specialized model for each camera. The main contribution of the paper is the development of a framework to assist in the automatic specialization of models for edge cameras. This framework aims to automatically increase the accuracy of the embedded models while optimizing the bandwidth during the process. 
    \item[A] \textit{Ekya: Continuous learning of video analytics models on edge compute servers}\cite{bhardwaj2022ekya} : The authors present a framework where the edge servers will jointly support inference and retraining task in order to handle the data drift of deployed compressed models. They express this problem by defining a performance metric by combining the precision of deployed models and eventually find an optimal scheduler. They also study the influence of context variation including lighting, class distribution, object count and camera location.
    
    \item[A]\textit{Unsupervised Multi-Target Domain Adaptation Through Knowledge Distillation}
\end{itemize}


\subsection{Accuracy vs efficiency online distillation}
% keywords - maximizing information online distillation
% distillation for video surveillance
% parsimonious knowledge distillation




\subsubsection{Delta Distillation for Efficient Video Processing}
In \cite{delta_distillation_2022}, they propose 

Let $x$ is the input, $f_\theta(x)$ and $g_\phi(x)$ is respectively a teacher and a student  parametric bloc. 

In , 

the main contribution is the replacement of the teacher's parametric bloc $f_\theta(x) $ in the classical distillation objective 
\begin{equation}
    L_d(x;\phi) = \mathrm{E}_x\left[||f_\theta(x)-g_\phi(x)||_2\right]
\end{equation}

Where, . 

By a term based on the temporal inter-frame difference in the output of the parametric bloc $z$, namely : 
\begin{equation}
    z_t = z_{t-1} +\Delta z_t
\end{equation}

We note that if two frames are identical, $\delta z_t$ is zero.

==> 4_SOTA/archives/main_sota.tex <==
\subsection{Deep-learning in edge constraints}
Deep-neural networks models (DNNs) are effective in several digital image processing applications (e.g.,industrial control, smart mobility, medicine). DNNs are able to directly process the images from an initial learning database and to generalize the distribution of the occurrence of a particular event. Therefore, when presented a new case, it estimates the probability of its occurrence. The DNNs analyse characteristics extracted automatically from their deep features, liberating the need of a manual intervention. They obtain, thanks to the predictive power of deep features, excellent results (accuracy, robustness to noise and good generalization on a variety of data).
\subsubsection{Scalability issues in model training}
Recent state-of-art models demonstrated impressive performance often at high-cost. Indeed, the training of large-scale DNNs requires high-performance cloud servers with a large-scale dataset which takes $i)$ many human labor resources to prepare the dataset or the training implementation, $(ii)$ a large amount of time and money cost. These costs are often prohibitive for most practitioners and hardware \cite{LucasBeyer2022}. Furthermore, a unique model with a single-training is not robust with respect to stochastic and ever-evolving environments. In the example of CCTV monitoring traffic at city-scale, there is no dataset large-enough covering all aspects of every urban landscape \cite{soviany2021curriculum}. Consequently, without regular domain adaptation models' performances \textbf{will eventually drop}.

\textcolor{red}{\textbf{To be integrated} Communication among servers is the limiting factor
to the scalability of distributed CNN training. For distributed data-parallel training, communication overhead is directly proportional to the number of parameters in the model (Iandola et al., 2016). In short, small models train faster due to requiring less communication. https://arxiv.org/pdf/1602.07360.pdf}

\subsection{Robust active learning}
Knowledge Distillation (KD) is a general approach promising a lightweight powerful models. The process assumes that, for the same dataset, large models (i.e, \emph{teacher}) have higher knowledge capacity than smaller models (i.e., \textit{students)}. The teacher can be a pre-trained model or a very large generic one such as GPT-3 and which can transfer the knowledge (i.e., pattern recognition mechanisms) to students without loss of validity. Other than Model Compression (MC), KD can be used for Unsupervised Domain Adaptation (UDA). UDA aims at preventing the performance’s loss of a model when it infers on a dataset distributed differently than the source domain. To improve its efficiency, recent direction \cite{rivas2022towards,delta_distillation_2022} attempt to exploit the contextual features of the scene to develop effective KD. They directly worked on the distillation scheme to develop more specialized students. For instance, in \cite{delta_distillation_2022}, they added a temporal dimension such that the student learns the variations in the teacher’s intermediate features over time. They thus take into account frame redundancies within a CCTV-stream. We claim that instead of working on the distillation scheme, a more \textbf{robust} and \textbf{scalable} approach involve an active learning. Assuming we are able to collect a sample of data from the target domain, a teacher is able to provide annotations from which the students can learn. This approach could help thus bridge the performance gap between large-scale models and affordable versions \cite{LucasBeyer2022}. 

 




Recent works \cite{rivas2022towards,delta_distillation_2022} exploits the contextual features of the scene to develop effective KD. For instance, in \cite{delta_distillation_2022}, they added a temporal dimension such that the student learns the variations in the teacher’s intermediate features over time. They thus take into account frame redundancies within a CCTV-stream. This does not take into account continual learning. 
\input{4_SOTA/ActiveLearning}
\input{4_SOTA/KnowledgeDistillation}

==> 4_SOTA/archives/related_work_AL.tex <==
\subsection{Active Learning} \label{sec:sota_al}

\acs{AL} enables efficient model development by reducing the number of labeled examples required to achieve satisfactory predictive performance \cite{Settles2009}. It is particularly valuable in computer vision, where data annotation is costly and time-consuming. Additionally, \acs{AL} curtails computational costs by retaining a representative subset, thus reducing the need to store and process extensive datasets. Three primary macro-scenarios are identified within \acs{AL}: membership query synthesis, pool-based \ac{AL}, and stream-based \ac{AL} \cite{OALSurvey}. While stream-based \ac{AL} is particularly pertinent to the current study, it has been mostly studied for classification and regression models \cite{SBAL,ROAL,ICML_SBAL}. We hereby provide an overview of \ac{AL} approaches for computer vision, distinguishing between methods specifically suited for image classification and object detection.

\subsubsection*{\acs{AL} for Image Classification}
Uncertainty-based strategies are key components of several \acs{AL} methods for image classification, employing techniques such as entropy \cite{Shannon1948}, margin-based sampling \cite{Roth2006}, Monte Carlo dropout \cite{Gal2017}, and ensemble methods \cite{Mohamadi} to estimate the uncertainty in model predictions. Alternatively, diversity-based strategies like Core-set \cite{Sener2017} aim to collect a diverse or representative set of observations. Hybrid strategies thrive to strike a balance between uncertainty and diversity. Notable examples include BADGE \cite{Ash2019}, CM \cite{Citovsky2021}, DSMRS \cite{Elhamifar2013}, CDAL \cite{Agarwal2020}, and CLUE \cite{Prabhu}. VAAL \cite{sinha2019variational} is another strategy that employs variational autoencoders for instance mapping into a latent space, letting a discriminator differentiate labeled from unlabeled samples. LLAL \cite{Yoo2019} is a task-agnostic strategy that introduces a loss prediction module to identify data points that the model is likely to misclassify. However, these approaches can hardly be generalized to the stream-based setting as they require expansive computation to evaluate the whole pool of observations before deciding which examples should be labeled. The few existing works on stream-based \acs{AL} for image classification leverage traditional statistical models \cite{ROZANEC2022277,Narr2016} and thus, do not provide a generalizable framework for large \acp{DNN}. Saran et al. \cite{saran23a} recently introduced the VeSSAL strategy for \acp{DNN} using volume sampling. They recommended a sampling probability for examples at time $t$, based on their gradient's contribution to the Fisher matrix. Unlike active distillation, this method relies on a perfect oracle for true labels.

\subsubsection*{\acs{AL} for Object Detection}
Roy et al. \cite{RoyUnmesh} classified \acs{AL} strategies for object detectors into two classes: white-box methods, reliant on network architecture, and black-box methods, based on informativeness scores like the confidence obtained from the softmax layer of the network. For black-box methods, aggregating confidence scores in multi-instance frames is challenging. A solution is the minmax strategy \cite{RoyUnmesh}, using the highest confidence score from detected bounding boxes. \cite{Brust2018} evaluated difference aggregation functions such as sum, average, and maximum when using the margin score in the multi-class setting. Finally, Aghdam et al. \cite{Aghdam2019} proposed a function to score the importance of each pixel and obtain an image-level metric by aggregating pixel-level scores. Alternative approaches rely on the use of ensemble to quantify model uncertainty.Feng et al. \cite{FengDi} introducing an \acs{AL} method for LiDAR 3D object detection using Monte Carlo dropout and deep ensembles. Schmidt et al. \cite{Schmidt2020} explored ensemble-based 2D object detection AL, introducing a consensus score for localization uncertainty and, drawing inspiration from \cite{Kao2018}, compared RoI proposals using an IoU matrix. Choi et al. \cite{DBLP:journals/corr/abs-2103-16130} addressed the computational costs of uncertainty estimation by proposing a strategy based on mixture density networks that estimates probabilistic distributions for localization and classification outputs. Yu et al. \cite{WeipingYu} introduced CALD, a consistency-based active learning strategy for object detection that integrates box regression with classification. It emphasizes consistency between original and augmented images and adjusts class distribution to address imbalances.

Similar to image classification, several methods combine uncertainty and diversity. Wu et al. \cite{WuEntropy} assess image uncertainty using entropy and target both intra-class and inter-class diversities with class-specific prototypes. Yang et al. \cite{Yang2022} introduced the PPAL algorithm, which blends uncertainty and diversity using features like difficulty-calibrated uncertainty and category-conditioned similarity. Yuan et al. \cite{Yuan2021} presented the MIAL framework, transitioning from instance-level to image-level uncertainty by filtering noise. It emphasizes informative instances and gauges single-image uncertainty by adjusting individual instance weights. Huang et al. \cite{Huang2022} introduced a frequency domain-based image selection method, emphasizing high-frequency regions for enhanced edge diversity. Beck et al. \cite{beck2023streamline} examined vehicular camera-collected images, devising a strategy to diversify data by prioritizing underrepresented scenarios, like foggy or rainy conditions, where the model struggles. While these approaches provide interesting insights into \acs{AL} for object detection, in most of the cases they cannot be directly applied to the stream-based framework. 

Recently, Arrotta et al. \cite{arrotta2023selfact} introduced SelfAct, a method combining self-supervision and streaming \acs{AL} for Human Activity Recognition models. They pre-train using self-supervision offline, followed by fine-tuning with \acs{AL} acquired labels. They used a sampling strategy aimed at collecting labels of data points that are deemed to be representative of a cluster. Self-labeling has also been used by Vaquet and Hinder \cite{vaquet2023combining}. They developed an \acs{AL} strategy for an incremental $k$-nn classifier that selects the examples to be pseudo-labeled when they have a high certainty and queries the ground truth when the mean certainty observed over a fixed time window drops below a pre-defined threshold.





==> 4_SOTA/archives/related_work_KD.tex <==
Active distillation is a paradigm in machine learning that aims to minimize the number of queries to teacher pseudo-labels, with the goal of fine-tuning a student model in a computationally and financially efficient way \cite{baykal2022robust}. This approach can be viewed as a synergistic melding of KD and AL methodologies. In light of this, we present a review of the latest advancements in these two research domains that pertain directly to our topic of interest. Furthermore, we offer insights into research that leverages clustering techniques within the realms of video analysis and multi-camera systems.

\subsection{Knowledge Distillation}

\acs{KD} is a strategy aimed at improving the efficiency of \acs{DNN} models without sacrificing their performance. This method, initially proposed by Hinton et al. \cite{hinton2015distilling}, facilitates the transfer of knowledge from a larger, more complex model, known as the teacher model, to a smaller, less resource-intensive model, referred to as the student model. The primary objectives of \acs{KD} are two-fold. The first goal, unsupervised domain adaptation, is to ensure that the student model continues to perform effectively even when operating on datasets with a different distribution from its training source \cite{saito2019semi}. This capability is crucial when the model is deployed in real-world situations where the data might vary from the original training data. The second objective, model compression, is to create lightweight models that are better suited to environments with constrained storage and computational capacities, such as mobile devices or embedded systems \cite{cheng2017survey}. By compressing a large model into a smaller one, \acs{KD} allows for the deployment of machine learning models in such resource-constrained settings, widening the application scope of artificial intelligence. The effectiveness of the \acs{KD} process can be influenced by several factors, including the relative sizes of the student and teacher models, the complexity of the task, the amount of available data, and the type of distillation method employed. Therefore, understanding these factors and how they interact is a significant area of ongoing research \cite{Furlanello2018, Tung2019}. In essence, KD represents a balance between model size and performance, and further research is needed to fully understand and optimize this trade-off. In this evolving landscape, recent advancements such as Online Distillation \cite{cioppa2019arthus, mullapudi2019online}, and Context-aware Distillation \cite{rivas2022towards, delta_distillation_2022} have further expanded the horizons of \acs{KD}. These pioneering approaches provide promising avenues for overcoming \acs{KD} inherent challenges, developing more efficient knowledge transfer techniques, enhancing the performance of smaller models, and enabling real-time adaptation to data distribution variations.


==> 4_SOTA/archives/sota_recup.tex <==
The idea is to use a trained teacher model and to distill its knowledge into the student model by guiding the student during the learning phase. A KD process can have two purposes: Unsupervised Domain Adaptation (UDA) \cite{oza2021unsupervised} and model compression.\\

UDA is a set of techniques to address the difficulties faced by a model in maintaining respectable accuracy when inferring on a dataset which is described by a significantly different data distribution compared to the source domain. In \cite{soviany2021curriculum} they argue that there is no dataset large enough to cover all aspects of an urban city scenario, and therefore a general-purpose detector may produce poor performance on the target set if the model is not adapted. Some works focus on incrementally enhancing the performance of a object detector over the target set by considering the model predictions as noisy and iteratively eliminating false positives and false negatives \cite{khodabandeh2019robust}\cite{li2021free}\cite{inoue2018cross}.\\

Other works propose methods to adapt a general purpose detector to a target video sequence such as in \cite{xu2019self} where the approach allows models to learn domain-invariant features for semantic segmentation through an attention mechanism that forces the student network to focus on discriminant features. In \cite{kang2017noscope} they propose a two step approach to first extract vehicle images in a video using a difference detector and then employ a student network to classify the image content. A heavy teacher network provides supervision to both the difference detector and the classifier. The authors in \cite{mhalla2016faster} propose to specialize a generic detector such as Faster R-CNN by utilizing a sequential Monte Carlo filter to adapt the detector to an unlabeled target video sequence. The training set generation is supported by the filter which considers the teacher predictions as samples from an unknown distribution. The false positives and false negatives are gradually eliminated by defining a likelihood function.\\ 

Model compression is of interest when looking at real-time applications and model integration for edge computing. One of the main problems with model compression is the severe limitation of the shallow model, the student, to perform as well as the teacher's model on the same dataset. This may be due to the fact that the student's network has difficulty constructing feature maps that are as discriminating as the teacher network to cope with the intricacies of the data distribution \cite{rivas2022towards}. However, a camera could be considered to observe only a small subset of a large data distribution in the context of a large-scale deployment \cite{bhardwaj2022ekya}. In \cite{shen2017fast} the authors proposes to skew the class distribution of large dataset by considering short-term distributions, which can be processed by simpler models due to the small number of classes. To this end, they implement a model selection policy by minimizing the processing time while maintaining the accuracy above a given threshold. This approach requires only one offline training, as in \cite{cai2019once} where a general-purpose deep network is trained before generating shallower networks via network pruning in order to be deployed in specific hardware configuration without retraining. This approach is effective in reducing the training cost of a large-scale deployment and addressing the hardware constraint by including it in the loop, but the domain shift issue is not mentioned in this work.\\

Specializing the model can also be done in a online fashion. This is the case of \cite{cioppa2019arthus} where the authors design a online knowledge distillation scheme in order to perform real-time human segmentation in sports videos. A light-weight model is progressively trained on a live video sequence through a heavy teacher model. The student performs the inference in real time while its weights are often updated by a offline student-teacher framework. Experiments show the model's ability to adapt to variations in context and ultimately appears to outperform its teacher. Online distillation is also employed in \cite{mullapudi2019online} to adapt a low-cost semantic segmentation model to a target video where the data distribution is not necessarily stationary. The student model appears to exhibit better temporal stability than the teacher model.\\ 

The latest research suggests that the use of prior knowledge about a scene and broadly speaking its contextual features could lead to inexpensive and more specialized students \cite{rivas2022towards}. While the paper does not specify which features, we claim that their position constitute an interesting research direction. As an example, \cite{delta_distillation_2022}, suggests that adding a temporal dimension benefit the knowledge distillation. In their proposal, the student learns the variations in the teacher’s
intermediate features over time. They demonstrate thus that these temporal variations can be effectively distilled due to the temporal redundancies within video frames. An alternative way of looking at the problem is that not every frame is relevant for learning. However, the assumption is valid, there is no work at the best of our knowledge that studies whether it is beneficial for a student to learn at fixed, random or criteria-based rates. In particular, would a student better learn if it's trained i) every deterministic \textit{K} frames, ii) $K \sim  \mathcal{N}(\mu,\,\sigma^{2})$ or iii) criteria as the presence of object's of interested or variation of illumination. 

